Active Imitation Learning from Multiple Non-Deterministic Teachers: Formulation, Challenges, and Algorithms

We formulate the problem of learning to imitate multiple, non-deterministic teachers with minimal interaction cost. Rather than learning a specific policy as in standard imitation learning, the goal in this problem is to learn a distribution over a policy space. We first present a general framework that efficiently models and estimates such a distribution by learning continuous representations of the teacher policies. Next, we develop Active Performance-Based Imitation Learning (APIL), an active learning algorithm for reducing the learner-teacher interaction cost in this framework. By making query decisions based on predictions of future progress, our algorithm avoids the pitfalls of traditional uncertainty-based approaches in the face of teacher behavioral uncertainty. Results on both toy and photo-realistic navigation tasks show that APIL significantly reduces the numbers of interactions with teachers without compromising on performance. Moreover, it is robust to various degrees of teacher behavioral uncertainty.

==> legacy_sections/formulation.tex <==

Our approach trains a query policy that issues a minimal number of queries that enable the agent to make a certain level of progress in getting closer to the goal set. 
Specifically, we denote by $\proset$ the set of states from which, if the agent continues following its current policies, the distance to the goal set will (in expectation) decrease at least by a factor of a pre-defined constant $\sigma$
\begin{align}
    \proset = \{  s \mid \exists j \in \mathbb{N}: j \geq 0 \wedge d(s) \geq \sigma \cdot  \bar{d}(s_{\rightarrow j}^{\hat{\pi}}) \}
    \label{eqn:proset}
\end{align} where $\bar{d}_{\tau}(s_{\rightarrow j}^{\hat{\pi}})$ is expected distance to the goal set $S^{\tau}_{\textrm{goal}}$ if the agent starts from state $s$ and follows policy $\hat{\pi}$ for $j$ steps. 

We formulate the learning problem of the query policy as the following optimization problem 
\begin{align}
    &\min_{\askpol} \ \mathbb{E}_{s \sim \mathbb{P}_{\hat{\pi}}, \hat{a}^{\textrm{ask}} \sim \askpol(z_s)} \left[ \ell_{\textrm{active}}(s, \hat{a}^{\textrm{ask}}) \right] \label{eqn:query_min}
    %& \text{s.t.} \  \forall \tau: \mathbb{P}_{\tau, \hat{\pi}}(s) = 0, s \notin \proset 
\end{align} where
\begin{align}
    \ell_{\textrm{active}}(s, \hat{a}^{\textrm{ask}}) = \mathds{1}\{ \hat{a}^{\textrm{ask}}_s = \texttts{query}\}^{\mathds{1}\left\{ s \in \proset \right\}}
    \label{eqn:active_loss}
\end{align}

%Note that the size of $\proset$ depends on the agent policies: the set expands if either (a) $\exepol$ becomes more effective or (b) $\askpol$ makes more queries to the teacher (and thus uses the teacher action to act more often). 
%Each state in $\proset$ is called a progressable state. 

In any state, this objective minimizes either query count or performance.
Consider two cases:
\begin{itemize}
    \item $s \in \proset$: $\ell_{\textrm{active}}(s, \hat{a}^{\textrm{ask}}) = \mathds{1}\{ \hat{a}^{\textrm{ask}}_s = \texttts{query}\}$. The objective directly minimizes the expected query count in $s$. 
    \item $s \notin \proset$: $\ell_{\textrm{active}}(s, \hat{a}^{\textrm{ask}}) = 1$. In this case, the agent receives a constant loss in $s$ regardless of the decision of the query policy.
    The agent can minimize this loss in expectation by (a) diminish the probability of visiting $s$ or (b) improving its policies $\hat{\pi}$ so that $s \in \proset$. 
\end{itemize}

The proposed problem formulation drives the behavior of the agent as follows. 
At the early stage of learning, when the agent has not learned from sufficient samples, it is incapable of satisfy the progress condition in most states. 
To avoid violating the condition, the agent needs to improve its execution policy by querying the teacher. 
In our setup, querying the teacher enhances performance of the agent in two ways: by acting with reference actions (short-term) and by imitation learning (long-term).
As the execution policy improves and helps the agent satisfy the progress condition in a state, the training objective shifts to query-count minimization in that state, forcing the query policy to reduce the number of queries.


The progress condition plays an important role in our formulation. 
First, it ensures the agent achieving a certain level of performance before starting to refrain from querying the teacher. 
Without this condition in the objective, the agent would trivially choose to avoid learning from the teacher to minimize the query count. 
Second, the progress condition integrates planning into the agent's decision-making process, as it is determined not by immediate behavior of the agent in the current time step, but by future outcomes realized by the agent policies. 


\noindent\textbf{Approximate verification of progress condition}. Deciding whether a state has satisfied the progress condition is intractable because of the dependency on the stochasticity of the agent policies and the environment dynamics. 
Our solution is to use sampled trajectories to construct an approximation of $\proset$ that can easily be verified membership of.

Formally, let $D$ be a set of trajectories drawned from the agent policies $\hat{\pi}$. 
Each trajectory $\zeta \in D$ has the form
\begin{align}
    (s_0, \hat{a}_0, s_1, \hat{a}_1, \cdots, s_n )
\end{align} where $\hat{a}_t = (\exea, \aska)$ and $n \leq T$.

We construct $\prosetapp$, an approximation of $\proset$, as follows
\begin{align}
    \prosetapp = \nonumber \{ & s_t \in \zeta \mid 
    \exists j, k \in \mathbb{N}: t \leq j < k \leq n \ \wedge \\
    &\hat{a}^{\textrm{ask}}_j = \texttts{query} 
    \wedge \hat{a}^{\textrm{ask}}_k = \texttts{query} \ \wedge \nonumber\\
    & d(s_j) \geq \sigma \cdot d(s_k) \}
    \label{eqn:prosetapp}
\end{align} 
Essentially, when the agent is in state $s_t$, it will look into the future states in the sampled trajectory to determine if the distance to the goal set will ever be reduced by more than a factor of $\sigma$.
We then substitute $\proset$ with $\prosetapp$ in the progress condition of \autoref{eqn:active_loss}.


Formally, let $\zeta = (s_0, \hat{a}_0, s_1, \hat{a}_1, \cdots, s_n )$ be a trajectory obtained by executing the agent policies $\hat{\pi}$, where $\hat{a}_t = (\exea, \aska)$ and $n \leq T$.
We construct $\prosetapp$, an approximation of $\proset$, as follows
\begin{align}
    \prosetapp = \nonumber \{ & s_t \in \zeta \mid 
    \exists j, k \in \mathbb{N}: t \leq j < k \leq n \ \wedge \\
    &\hat{a}^{\textrm{ask}}_j = \texttts{query} 
    \wedge \hat{a}^{\textrm{ask}}_k = \texttts{query} \ \wedge \nonumber\\
    & d(s_j) \geq \sigma \cdot d(s_k) \}
    \label{eqn:prosetapp}
\end{align} 
Essentially, when the agent is in state $s_t$, it will look into the future states in the sampled trajectory to determine if the distance to the goal set will ever be reduced by more than a factor of $\sigma$.
We then substitute $\proset$ with $\prosetapp$ in the progress condition of \autoref{eqn:active_loss}.




==> legacy_sections/method.tex <==
\newcommand{\algopar}{\par\hskip\algorithmicindent}

We present an imitation learning-based solution to the optimization problem introduced in the previous section. 
To motivate our approach, we rewrite the objective in \autoref{eqn:query_min} as 
\begin{align}
    \min_{\askpol} \ &\sum_{s^{\odot} \in \proset} P_{\hat{\pi}}(s^{\odot}) \askpol(s^{\odot}, \texttts{query}) + \nonumber \\ 
    &\sum_{s^{\otimes} \notin \proset} P_{\hat{\pi}}(s^{\otimes})
\end{align}

Here, the first term minimizes the probability of querying in states of $\proset$, while the second term minimizes the chance of visiting states of $\badset$.

We consider the two term separately and define a query policy that effectively minimizes each term.
It is easy to see that the first term achieves a minimum value (of 0) with a query policy that always selects the \texttts{continue} action. 
In contrast, assuming the execution teacher is optimal, the minimizer of the second term is a policy that always chooses to \texttts{query}, because an agent equipped with this query policy always acts with (optimal) execution actions. 
Even when the execution teacher is not optimal but substantially more competent than the agent, such a query policy is still a decent solution for the second term.
Hence, we define a query teacher $\askexp$ as follows
\begin{align}
    \askexp(s) = \begin{cases}
    &\delta_{\texttts{continue}} \ \ \text{if } s \in \proset \\
    &\delta_{\texttts{query}} \ \ \ \ \ \  \text{if } s \notin \proset \\
    \end{cases}
\end{align} where $\delta_a$ is a delta distribution that assign a probability of 1 to a single action $a$.

We then teach the query policy to imitate the query teacher under a standard imitation learning objective 
\begin{align}
    \min_{\askpol} \mathbb{E}_{s \sim \mathbb{P}_{\hat{\pi}}}\left[ \ell_{\textrm{CE}}(s, \askpol, \askexp) \right]
\end{align}

It is important to emphasize that, unlike that the execution teacher, the cost of querying the query teacher is substantially small  






\begin{algorithm}[tb]
\caption{Hindsight Active Imitation Learning (HAIL)}
\label{alg:main_algo}
\begin{algorithmic}[1] %[1] enables line numbers
\STATE \textbf{Input}: task command $c_q$ and start state $ s_{\textrm{start}}^q$ 
\STATE execute \autoref{alg:active_task_exe} with current policies $\hat{\pi}$ to receive 
\begin{itemize}
    \item trajectory $\tau = (s_0, \hat{a}_0, s_1, \hat{a}_1, \cdots, s_T ) $ where $\hat{a}_t = (\exea, \aska)$;
    \item distances to goal set $\{ d(s_t) \mid \aska = \texttt{ask} \}$.
\end{itemize}
\FOR{$t = 0 \cdots T - 1$}
\STATE construct $\prosetapp$ according to \autoref{eqn:prosetapp}
\STATE compute $a^{\textrm{ask}\star}_t$ using \autoref{tab:query_teacher}, replacing $\proset$ with $\prosetapp$
\STATE compute imitation loss $\ell_q^{\textrm{ask}}(s, \askpol, \askexp) $
\ENDFOR
\STATE update $\askpol$ by minimizing \autoref{eqn:query_obj}

\end{algorithmic}
\end{algorithm}

\noindent\textbf{Final algorithm}. \autoref{alg:main_algo} summarizes our training algorithm, named \emph{Hindsight Active Imitation Learning} (HAIL). 
The algorithm first calls \autoref{alg:active_task_exe} with the current query policy to optimize the execution policy and obtain a sample trajectory. 
Next, it revisits the states in the sample trajectory and computes the query teacher action in each state. 
Finally, it teaches the query policy to imitate the actions suggested by the query teacher. 
To reduce computational cost, we introduce a new mode of agent-teacher communication, called \emph{hindsight teaching}, that enables all time steps to share a single sample for approximating of $\proset$. 
In this approach, the teacher does not compute a decision in state on-the-fly, within the time step it is queried.
Instead, the query teacher waits until the agent terminates and then retroactively decides the $\prosetapp$-membership of each state $s_t$.
This mode of communication is not modeled by conventional imitation learning setups, where the teacher policy is assumed to be independent of the agent policy and thus can compute a reference action within a current time step.
In our case, because the query teacher teaches the agent only after the entire trajectory has been generated, we call this mode of communication hindsight teaching. 

==> legacy_sections/old_exp_setup.tex <==
\begin{figure*}[t!]
\centering
\begin{subfigure}{.33\linewidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{images/str_dev_curve.pdf}  
  \caption{\strprob}
  \label{fig:pos_dev_perform}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/pos_dev_curve.pdf}  
  \caption{\posprob}
  \label{fig:vln_dev_perform}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/vln_dev_curve.pdf}  
  \caption{\vlnprob}
  \label{fig:vln_dev_perform}
\end{subfigure}
\caption{Performance against number of queries to teacher on validation data. Methods: behavior cloning (BC), full imitation learning (FIL), error-based (ERR), and hindsight active imitation learning (HAIL; our method).} 
\label{fig:dev_perform}
\end{figure*}




\begin{table}[t!]
    \small
    \centering
	\begin{tabular}{lcccc}
		\toprule[1pt]
		  & \strprob & \posprob & \vlnprob \\
		 \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
		Dataset & Synthesized & CITE & CITE  \\
		Training size & 8,000 & 12,543 & 14,039  \\
		Development size & 1,000 & 2,002 & 2,349  \\
		Test size & 1,000 & 2,077 & 4,173  \\
		Execution actions & 5 & 18 & 37 \\
		Batch size & 32 & 128 & 32 \\
		Learning rate & $10^{-3}$ & $10^{-3}$ & $10^{-4}$ \\
        \bottomrule[1pt] 
	\end{tabular}
	\caption{Data statistics of three experimented problems: string expansion (\strprob), English \posprob tagging (\posprob), and vision-language navigation (\vlnprob).}
	\label{tab:data}
\end{table}

We conduct experiments on three problems: string expansion (\strprob), English part-of-speech tagging (\posprob), and vision-language navigation (\vlnprob). 
These problems represent environments of diverse complexity, where \strprob features a simple toy environment and \vlnprob presents a complex multimodal environment. 
\autoref{tab:data} summarizes the datasets we use for these problems. 

\noindent\textbf{String expansion} (\strprob). The input of the agent is a string $(d_1, w_1, d_2, w_2, \cdots, d_n, w_n)$, which encodes Latin alphabetic characters $w_i \in \{\texttt{A}, \texttt{B}, \texttt{C}, \texttt{D}\}$ and numbers of times they repeat $d_i = \{\texttt{1}, \texttt{2}, \texttt{3}, \texttt{4}, \texttt{5}\}$.
The agent must output a string in which each character $w_i$ repeats $d_i$ times and the characters preserve their order as in the input string. For example, an input \texttt{2A4B3C} maps to the output \texttt{AABBBBCCC}. 
Each input string contains from 3 to 7 alphabetic characters. 
The output action space is the characters from \texttt{A} to \texttt{D} and a special \texttt{EOS} token. 

\noindent\textbf{English part-of-speech tagging} (\posprob). Given an English sentence, $(w_0, w_1, \cdots, w_{n - 1}, w_n)$, the agent has to generate the task sequence $(y_0, y_1, \cdots, y_{n - 1}, y_n)$ where $y_i$ is the part-of-speech tag of word $w_i$.
We use the Universal Dependencies English Web Treebank version 2.5 provided by CITE.
The execution action space consists of 17 standard Universal Dependencies \posprob tags and a special \texttt{EOS} tag. 

\noindent\textbf{Vision-language navigation} (\vlnprob). In this problem, an agent navigates in a photorealistic environment by following an English instruction given by a human. 
The instruction is a sequence of words $(w_0, w_1, \cdots, w_n)$, which the agent takes as input to generate a sequence of navigation actions $(a_0, a_1, \cdots, a_m)$.
We use the \vlnprob photorealistic simulator and the Room-to-Room dataset (CITE Anderson).\footnote{The original dataset provide evaluation sets with seen and unseen environments. We report evaluation results only on unseen environments in this paper.}
Walking in the environment is modeled as traversing in an undirected graph, whose edges connect locations that are nearby and walkable from one another. 
Following CITE speaker-follower, we employ a panoramic action space that divides the panoramic of the agent into 36 actions that correspond to 36 view angles. 
At every time step, the agent chooses a next location and maps it to the closest view angle.
It then rotates toward that view angle and walks straight to the chosen next location.
A special \texttt{STOP} is added to signal when the agent wants to terminate.

\noindent\textbf{Execution policy}. The \strprob execution policy is an LSTM-based encoder-decoder model with a hidden size of 32 and an input word embedding size of 16.
The \posprob execution policy is a bidirectional LSTM with a hidden size of 128 and a word embedding size of 64. 
The \vlnprob execution policy is adapted from the Transformer-based encoder-decoder model developed by CITE Hanna. 

\noindent\textbf{Evaluation metrics}. For \strprob and \posprob, we compute the accuracy of the predicted sequence, i.e. the fraction of time steps on which the agent generated correct output tokens. 
For \vlnprob, the agent is considered as successfully fulfilled an instruction if after $T$ time steps it stands within 3 meters of the target location referenced by that instruction. 
We report success rate, the fraction of instructions that are successfully fulfilled. 

\noindent\textbf{Query policy}. The query policy follows the same design in all problems. 
It is an LSTM model that has the same hidden size as that of the execution model. 
The input features of the query model at time step $t$ are: an embedding of of the previous query action, an embedding of the remaining time steps ($T - t$), the current hidden state output by the execution model, and the execution action probability distribution. 
We concatenate these features into a single vector and feed it into the LSTM query model. 
We do not back-propagate the query loss through the execution model's hidden state and action distribution.

\noindent\textbf{Training Hyperparameters}. We use Adam optimizer (CITE). 
Unless otherwise stated, we use $\sigma = 6$ in the HAIL algorithm. 
The time constraint is set to the length of the input sequence (in \strprob and \posprob) or 10 (in \vlnprob). See \autoref{tab:data} for more detail.

\textbf{Skylines}. We compare our method (HAIL) with the following skylines
\begin{itemize}
    \item Behavior cloning (BC): queries the teacher in every time step and always chooses the teacher action to act.
    \item Full imitation learning (FIL): also queries the teacher in every time step but uses the agent action to act. 
    \item Error-based policy (ERR): queries the teacher in time steps in which the agent action differs from the teacher action. We compare with this skyline to demonstrate that designing a good query policy is challenging even when we can perfectly predict when the agent makes mistakes. In addition, it also showcases the drawbacks of a myopic policy that only looks one-step ahead. 
\end{itemize}



==> legacy_sections/old_results.tex <==
\begin{figure}[t!]
\centering
\begin{subfigure}{.49\linewidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{images/total_query.pdf}  
  \caption{}
  \label{fig:total_query}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/ask_ratio.pdf}  
  \caption{}
  \label{fig:ask_ratio}
\end{subfigure}
\caption{(a) Total number of queries and (b) query ratio over time (each data point is the fraction of time steps on which the agent queries the teacher since the last data point is calculated).} 
\label{fig:dev_perform}
\end{figure}

\begin{figure}[t!]
\centering
\begin{subfigure}{.49\linewidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{images/sigma_acc.pdf}  
  \caption{}
  \label{fig:sigma_acc}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/sigma.pdf}  
  \caption{}
  \label{fig:sigma}
\end{subfigure}
\caption{(a) Success rate and (b) Query ratio over time of the HAIL agent on the \vlnprob development set.} 
\label{fig:sigma_effect}
\end{figure}

\begin{table}[t!]
    \small
    \centering
	\begin{tabular}{lccccccc}
		\toprule[1pt]
		 & \multicolumn{2}{c}{\strprob} & \multicolumn{2}{c}{\posprob} & \multicolumn{2}{c}{\vlnprob} \\
		 \multicolumn{1}{c}{Method} & Val & Test & Val & Test & Val & Test \\
		 \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}
		 \cmidrule(lr){6-7} 
		BC & 99.2 & 99.4 & 88.6 & 88.0 & 31.7 & 29.2 \\
		FIL & \textbf{99.7} & \textbf{99.7} & 88.8 & \textbf{89.0} & 36.5 & 31.5 \\
		ERR & 97.5 & 97.5 & 87.8 & 87.9 & 33.6 & 30.9 \\
		HAIL (ours) & 99.1 & 99.2 & \textbf{88.9} & 88.8 & \textbf{36.7} & \textbf{33.8} \\
        \bottomrule[1pt] 
	\end{tabular}
	\caption{Final performance on validation and test data. The best result in a column is in bold.}
	\label{tab:unseen_acc}
\end{table}

\noindent\textbf{Main results}. \autoref{fig:dev_perform} presents performance of the agent with different query policies on three problems. 
All agents in the same problem are trained on the same number of data batches. 
Results show similar trends in three problems.

First, the FIL agents are slightly better than the BC agents, especially on \vlnprob with a gap of +4.8\% on the development set. 
The ERR query policies issue fewer queries compared to other policies. 
The agents equipped with this policy learn more quickly at the beginning of training but achieve lower accuracy (or success rate) overall. 
On \vlnprob, the ERR agent is outperformed by the FIL agent by 2.9\% on the development set. 
On \strprob and \posprob, this agent achieves worst performance among all agents.
These results show that only learning to correct mistakes may not be sufficient to achieve high performance.
Even when the agent behaves optimally in a situation, it may need extra supervision to reduce uncertainty in its decisions. 

Our method (HAIL) attains performance comparable with BC and FIL on unseen data while using much fewer queries.
As seen in \autoref{tab:unseen_acc}, the gaps between HAIL and the best methods are less than 0.5\% on \strprob and \posprob.
On \vlnprob, HAIL even outperforms other methods on both validation and test data. 

\autoref{fig:total_query} shows the total number of queries made by each agent on the same number of data batches. 
On average, HAIL makes about three times fewer queries compared to FIL.
The HAIL query policy is less conservative than the ERR policy, issuing sufficient queries to avoid hurting generalization. 


\noindent\textbf{Does the query policy adapt to the capability of the execution policy?} In \autoref{fig:ask_ratio}, we plot the query ratio per episode, which is the fraction of time steps on which the agent chooses to query, over time.
We observe that in all problems, the query ratio decreases over time. 
Moreover, the decreasing rate correlates with the diffulty of the problem. 
For example, on \strprob, where the agent achieves almost perfect accuracy, the query ratio descreases dramatically from $~$50\% to $~$25\%.
In contrast, on the more complex \vlnprob problem, the query ratio only drops by 5.6\% throughout training.


\noindent\textbf{The effect of $\sigma$}. We investigate the effect of the hyperparameter $\sigma$ on the query ratio and the performance of the HAIL agent on the \vlnprob problem (\autoref{fig:sigma_effect}). 
We vary the value of $\sigma$ from 2 to 10. 
Overall, we observe that the learning rate of this agent is largely unaffected when $\sigma$ varies.
Smaller values of $\sigma$ forces the agent to make fewer queries. 


==> legacy_sections/problem.tex <==
In practice, the teacher is usually a human or a search algorithm, whose cost to compute decisions is expensive. 
Conventional imitation learning algorithms (CITE) incur maximum communication costs because they query the teacher in \emph{every} state the agent visits during training. 
The goal of active imitation learning (AIL) is to reduce the number of queries made to the teacher during training without degrading performance of the agent. 

Formally, in AIL, the agent maintains two policies: an execution policy $\exepol$ for executing a main task, and a query policy $\askpol$ for deciding when to query an execution teacher policy $\exeexp$. 
The query policy maps an observation $z_t$ and a task command $c^{\tau}$ to an action distribution over the query action space $A^{\textrm{ask}} = \{\texttts{continue}, \texttts{query}\}$. 
%At time step $t$, a query action $\aska$ is chosen by either sampling from or taking the highest-probability action of the distribution $\askpol(\cdot\mid z_t; c^{\tau})$. 
At time step $t$, the agent selects a query action $\aska \sim \askpol(z_t)$.
If $\aska = \texttts{query}$, the agent queries the teacher and receives a reference execution action $\exearef$.
It can then use this action to learn to better mimic the teacher.
In addition, the teacher also provides $d(s_t)$, the distance to the goal set from the current state.
If $\aska = \texttts{continue}$, the agent continues executing the task using its own execution policy without querying the teacher. 

Including distance-to-goal measurements in the teacher's responses differentiates our setup from previous work (CITE), where the teacher only provides reference actions. 
These measurements play an important role in our framework, as we use them to teach the agent to be aware of future consequences.
In any standard MDP, a simple distance metric can be defined as $d(s_t) = R^{\star} - \hat{R}_t$, where $R^{\star}$ is the final reward obtained by the teacher and $\hat{R}_t$ is the reward obtained by the agent at time step $t$.
In more specific domains, better-tailored metrics can be employed.
For example, in our experiments, we use shortest-path distance for a navigation task and Levenshtein string-edit distance for sequence-prediction tasks. 
Computing these metrics is cheap and does not require any additional information beyond information required to compute the reference execution actions. 



\begin{algorithm}[tb]
\caption{Active imitation learning with learned $\askpol$}
\label{alg:active_task_exe}
\begin{algorithmic}[1] %[1] enables line numbers
\STATE \textbf{Input}: $s_{\textrm{start}}$
\STATE set $s_0 = s_{\textrm{start}}$
\FOR{$t = 0 \cdots T - 1$}
\STATE observe $z_t \sim P_O(\cdot\mid s_t)$
\STATE choose a query action $\aska \sim \askpol(z_t)$
\IF{$\aska = \texttts{query}$}
\STATE query teacher to receive reference action $\exearef$ and distance to goal set $d(s_t)$
\STATE compute imitation loss $\ell_{\textrm{exe}}(s, \exepol, \exeexp)$
\STATE use reference action to act $\exea = \exearef$
\ELSE
\STATE use agent action to act $\exea \sim \exepol(z_t)$
\ENDIF
\STATE \textbf{if} {$\exea = \texttts{stop}$} \textbf{then break}
\STATE arrive in new state $s_{t + 1} \sim P_T(\cdot\mid \exea, s_t)$
\ENDFOR
\STATE update $\exepol$ by minimizing \autoref{eqn:active_exepol}
\end{algorithmic}
\end{algorithm}

\noindent\textbf{Learning $\exepol$ with fixed $\askpol$}. Introducing the query policy alters the objective for learning the execution policy in two ways. 
First, the agent-induced state distribution now depends on \emph{both} policies rather than on only the execution policy. 
Second, an execution imitation loss $\ell_{\textrm{CE}}(s, \exepol, \exeexp)$ is incurred only when the agent decides to query. 
We denote $\mathbb{P}_{\hat{\pi}}$ as the state distribution induced by $\hat{\pi} = (\exepol, \askpol)$.
The objective for learning $\exepol$ given a fixed $\askpol$ is 
\begin{align}
    \min_{\exepol} \mathbb{E}_{s \sim \mathbb{P}_{\hat{\pi}}, \hat{a}^{\textrm{ask}} \sim \askpol(z_s)}\left[ \ell_{\textrm{exe}}(s, \exepol, \exeexp) \right]
    \label{eqn:active_exepol}
\end{align} where \begin{align}
    \ell_{\textrm{exe}}(s, \hat{\pi}, \pi^{\star}) \equiv  \ell_{\textrm{CE}}(s, \hat{\pi}, \pi^{\star}) \cdot \mathds{1}\{ \hat{a}^{\textrm{ask}} = \texttts{query} \}
\end{align} with $\mathds{1}\{.\}$ being an indicator function that returns 1 if the logic inside the braces is true and returns 0 otherwise.

This objective differs from the training objective in conventional imitation learning (\autoref{eqn:orin_il}) only in the state distribution on which the imitation loss is averaged over. 
Hence, online learning-based imitation learning algorithms such as \textsc{DAgger} (CITE) or \textsc{AggreVaTe} (CITE) can be used to optimize the objective effectively, since these algorithms do not make any assumptions about the input data distribution. 

\autoref{alg:active_task_exe} demonstrates active imitation learning with a fixed, learned query policy. 
In general, every time the agent queries to the teacher, it can choose to use whether the newly received reference action or its own action to act in the environment. 
In this work, however, we assume the agent \emph{always} uses the reference action to act. 
This choice enables safer exploration during training, resulting in higher training performance and faster convergence. 

==> legacy_sections/teacher.tex <==
The standard I2L setup assumes that there is only a single teacher interacting with the agent. 
Moreover, even though not explicitly assumed, the teacher is usually deterministic, i.e. $\pi^{\star}(s)$ outputs a one-hot action distribution. 

We model the general case where the agent may interact with multiple teachers and the teachers may act stochastically. 
We define a teacher distribution $p^{\star}(\pi)$ over teacher policies.
At the beginning of each episode, a teacher policy $\pi^{\star}$ is re-sampled from $p^{\star}(\pi)$ and will interact with the agent throughout the episode. 
We are interested in two special cases of this setup
\begin{itemize}
    \item The agent interacts with a single, stochastic policy. In this case, the teacher distribution is a one-hot distribution but the mode policy is not. We called this teacher an erratic teacher. 
    \item The agent interacts with a mixture of deterministic policies. Each deterministic policy $\pi_i^{\star}$ has a probability of $\alpha_i$ to be drawn from the teacher distribution. We called this teacher a community teacher. 
\end{itemize}



==> legacy_sections/tmp.tex <==
In this approach, we construct two query teacher $\askexp$ and train the query policy to mimic its behavior via imitation learning. 
The query teacher is deterministic, i.e. it outputs an action distribution that assigns a probability of $1$ to a single action. 

To construct this teacher, we first introduce a special action $\texttts{ignore}$ into the query action space. 
When the teacher issues this action in a state, it does not want the agent to learn anything in that state. 
In other words, the query policy optimizes the following objective
\begin{align}
    \min_{\askpol} \mathbb{E}_{\tau \sim \mathcal{U}, s \sim \mathbb{P}_{\tau, \hat{\pi}}}\left[ \ell_{\tau}^{\textrm{ask}}(s, \askpol, \askexp) \right]
    \label{eqn:query_obj}
\end{align} where
\begin{align}
     \ell_{\tau}^{\textrm{ask}}(s, \hat{\pi}, \pi^{\star}) \equiv \ell_{\tau}^{\textrm{CE}}(s, \hat{\pi}, \pi^{\star}) \cdot \mathds{1}\{ a^{\textrm{ask}\star}_s \neq \texttts{ignore} \}
\end{align} with $ a^{\textrm{ask}\star}_s \mapsfrom \pi^{\textrm{ask}\star}(. \mid s; \tau)$ being the action suggested by the query teacher in state $s$.

Consider a trajectory $\zeta$ sampled from the agent's current policies. Suppose the agent takes action $\hat{a}^{\textrm{ask}}_s$ in state $s \in \zeta$.
The decision of the teacher depends on (a) the agent action $\hat{a}^{\textrm{ask}}_s$ and (b) whether it can meet the progress constraint in state $s$

\begin{table}[h!]
\centering
\begin{tabular}{lll}  
\toprule
\multicolumn{1}{c}{$\hat{a}^{\textrm{ask}}_s$}  & \multicolumn{1}{c}{$s \in \prosetapp$} & \multicolumn{1}{c}{$s \notin \prosetapp$} \\
\midrule
continue & continue  & query      \\
query & ignore  & continue       \\
\bottomrule
\end{tabular}
\caption{Action $a^{\textrm{ask}\star}_s$ suggested by $\askexp$ under different scenarios.}
\label{tab:query_teacher}
\end{table}

In other words,
\begin{itemize}
    \item If $s \notin \prosetapp$, the teacher \emph{disagrees} with the agent, suggesting the opposite action (i.e. $\texttts{query} \rightleftharpoons \texttts{continue}$);
    \item If $s \in \prosetapp$, the teacher \emph{agrees} with the agent, suggesting the same action except that, if the agent has chosen to query, the teacher is ignored.
\end{itemize}

%In practice, since the progress constraint cannot be verified efficiently, we use $\prosetapp$ instead of $\proset$ to compute the query teacher's decisions. 
%However, to provide insights into our algorithm that are independent of the approximation method, we will focus on proving several desirable properties of the hypothetical query teacher defined in \autoref{tab:query_teacher}.
%Specifically, we will show that mimicking this teacher helps the agent (a) meet the progress constraint if it has not and (b) reduce the number of queries if the agent has met the constraint. 

Next, we show that mimicking this teacher helps the agent (a) meet the progress constraint if it has not and (b) reduce the number of queries if the agent has met the constraint. 

Suppose that there exists a query action such that the agent will satisfy the progress constraint if it takes that action in the current state and continues acting using its own policies.
The following lemma shows that the query teacher always suggests that action. 

\begin{lemma}
Suppose, at time step $t$, the agent is in state $s$ and the query teacher suggests an action $a^{\star} \neq \texttts{ignore}$. For $a \in A^{\textrm{ask}} \setminus \{\texttts{ignore}\}$, let $\tilde{\pi}_{\textrm{ask}}[a]$  be a one-step deviation policy that chooses action $a$ in time step $t$ and follows the agent's query policy in subsequent time steps
\begin{align}
    \tilde{\pi}_{\textrm{ask}}[a] = \begin{cases}
    \delta_a \ \ & \text{at time step } i = t \\
    \askpol \ \ & \text{at time step $i$ for } t < i \leq T \\
    \end{cases}
\end{align} where $\delta_a$ is a delta distribution that assigns probability 1 to only action $a$. 

Let $\tilde{\pi}[a] = (\exepol, \tilde{\pi}_{\textrm{ask}}[a])$. 
Suppose there exists an action $\alpha \in A^{\textrm{ask}} \setminus \{\texttts{ignore}\}$ such that $s \in S^{\odot}_{\tilde{\pi}[\alpha]}$, i.e.
\begin{align}
    \exists j, k: \ 0 \leq j < k \wedge \bar{d}\left(s_{\rightarrow j}^{\hat{\pi}[\alpha]} \right) \geq \sigma \cdot \bar{d}\left(s_{\rightarrow k}^{\hat{\pi}[\alpha]} \right)
\end{align} 

Then, $s \in S^{\odot}_{\tilde{\pi}[a^{\star}]}$.
\end{lemma} 

\begin{proof} 
Let $\hat{a}$ be the query action taken by the agent in state $s$. We consider two cases:
\begin{itemize}
\item $s \in \proset$: by definition of the query teacher, $\hat{a} = a^{\star}$. Thus, $s \in S^{\odot}_{\tilde{\pi}[a^{\star}]}$.
\item $s \notin \proset$: by definition of $\alpha$, this implies that $\alpha \neq \hat{a}^{\textrm{ask}}_s$. Also, by definition of the query teacher, $a^{\star} \neq \hat{a}$. Since $\left|A_{\textrm{ask}} \setminus \{ \texttts{ignore} \} \right| = 2$, it must be the case that $\alpha  = a^{\star}$. Since $s \in S^{\odot}_{\tilde{\pi}[\alpha]}$, it follows that $s \in S^{\odot}_{\tilde{\pi}[a^{\star}]}$. 
\end{itemize}
\end{proof}

The next lemma explains the behavior of the query teacher when $s \in \prosetapp$.
It shows that, using a cross-entropy imitation loss (\autoref{eqn:cross_entropy}), the query policy's imitation learning objective (\autoref{eqn:query_obj}) shares the same gradient with respect to the agent's query policy with the query-minimization objective (\autoref{eqn:rl_obj}).
Thus, using gradient descent methods to optimize one also optimizes the other.
For notation brevity, we omit the dependency on the task $q$ in the lemma's statement and proof.

\begin{lemma}
Let $\mathcal{L}_{\textrm{imitate}}$ be the query policy's imitation learning objective in \autoref{eqn:query_obj} with a cross-entropy imitation loss (\autoref{eqn:cross_entropy})
\begin{align}
    & \mathcal{L}_{\textrm{imitate}}(\askpol) \equiv \nonumber \\ 
    &- \mathbb{E}_{s \sim \mathbb{P}_{\hat{\pi}}}\left[ \log \askpol(a^{\textrm{ask}\star}_s \mid z_s) \cdot [\![ a^{\textrm{ask}\star}_s \neq \texttt{ignore} ]\!] \right]
\end{align}

Let $\mathcal{L}_{\textrm{qmin}}$ be the query-minimization objective in \autoref{eqn:rl_obj}
\begin{align}
    \mathcal{L}_{\textrm{qmin}}(\askpol) \equiv \mathbb{E}_{s \sim \mathbb{P}_{\hat{\pi}}} \left[ [\![ a^{\textrm{ask}}_s = \texttt{ask} ]\!] \right] 
\end{align} 

When $s \in \proset$, we have
\begin{align}
    \nabla \mathcal{L}_{\textrm{imitate}}(\askpol) = \nabla \mathcal{L}_{\textrm{qmin}}(\askpol)
\end{align}
\end{lemma}

\begin{proof}
$\mathcal{L}_{\textrm{qmin}}(\askpol)$ can be rewritten as
\begin{align}
    \mathcal{L}_{\textrm{qmin}}(\askpol) 
    &= T -\mathcal{L}_{\textrm{reinforce}}(\askpol) \\
    &\equiv T - \mathbb{E}_{s \sim \mathbb{P}_{\hat{\pi}}} \left[ [\![  \hat{a}^{\textrm{ask}}_s \neq \texttt{ask} ]\!] \right]
    \label{eqn:rl_obj}
\end{align} 

Therefore, minimizing $\mathcal{L}_{\textrm{qmin}}$ is equivalent to maximizing $\mathcal{L}_{\textrm{reinforce}}$.
The objective
\begin{align}
    \max_{\askpol} \mathcal{L}_{\textrm{reinforce}}(\askpol) 
\end{align} can be viewed as a reinforcement learning problem with reward $r(s, a) = [\![ a \neq \texttt{ask} ]\!]$. 
We apply the policy gradient theorem (CITE) to derive the gradient of $\mathcal{L}_{\textrm{reinforce}}$ with respect to $\askpol$
\begin{align}
    &\nabla \mathcal{L}_{\textrm{reinforce}}(\askpol) = \nonumber \\ &\mathbb{E}_{s \sim \mathbb{P}_{\hat{\pi}}} \left[ \log \askpol(\hat{a}^{\textrm{ask}}_s \mid z_s) \cdot [\![ \hat{a}^{\textrm{ask}}_s \neq \texttt{ask} ]\!] \right]
    \label{eqn:policy_grad}
\end{align}

On the other hand,
\begin{align}
    &\nabla \mathcal{L}_{\textrm{imitate}}(\askpol) = \nonumber \\ 
    & - \mathbb{E}_{s \sim \mathbb{P}_{\hat{\pi}}} \left[ \log \askpol(\hat{a}^{\textrm{ask}}_s \mid z_s) \cdot [\![ a^{\textrm{ask}\star}_s \neq \texttt{ignore} ]\!] \right]
\end{align}

Notice that when $s \in \proset$, 
\begin{align}
    [\![ a^{\textrm{ask}\star}_s \neq \texttt{ignore} ]\!] = [\![ \hat{a}^{\textrm{ask}}_s \neq \texttt{ask} ]\!] 
\end{align}

Therefore,
\begin{align}
    \nabla \mathcal{L}_{\textrm{imitate}}(\askpol) = -\nabla \mathcal{L}_{\textrm{reinforce}}(\askpol) = \nabla \mathcal{L}_{\textrm{qmin}}(\askpol)
\end{align}
\end{proof}

==> sections/impact.tex <==
Current machine learning-based agents exhibit limited capabilities of interacting with humans. Most models operate in a passive way. When in trouble, they cannot reach out to external knowledge sources to acquire additional knowledge; to improve, these models must wait to be fueled with more data.
This work enables machine learning models to actively leverage diverse sources of knowledge available in the physical and virtual human world.
The application considered in this work, where an assistant robot follows natural language instructions to complete tasks, can potentially benefit people who cannot fully take care of themselves (e.g., the elderly or people with visual or motor impairments).  

Knowledge may vary across different sources.
If the agent is not well-equipped to capture this difference, it may be confused and release disastrous decisions. 
For example, in \cite{ke2019imitation}, a toy example is given where a self-driving is taught to get around an obstacle by either going to the left or the right of the obstacle. 
For multiple standard imitation learning approaches, the car learns an interpolation of the two directions and decides to go straight to the obstacle.
Such a scenario would lead to severe damage or even human deaths in the real world. 
The algorithm developed in this work mitigates this problem through learning representations that characterize individual sources of knowledge.
